Automated Extraction of Multicomponent Alloy Data Using Large Language Models for Sustainable Design

The design of sustainable materials requires access to materials performance and sustainability data from literature corpus in an organized, structured and automated manner. Natural language processing approaches, particularly large language models (LLMs), have been explored for materials data extraction from the literature, yet often suffer from limited accuracy or narrow scope. In this work, an LLM-based pipeline is developed to accurately extract alloy-related information from both textual descriptions and tabular data across the literature on high-entropy (or multicomponent) alloys (HEA). Specifically two databases with 37,711 and 148,069 entries respectively are retrieved; one from the literature text, consisting of alloy composition, processing conditions, characterization methods, and reported properties, and other from the literature tables, consisting of property names, values, and units. The pipeline enhances materials-domain sensitivity through prompt engineering and retrieval-augmented generation and achieves F1-scores of 0.83 for textual extraction and 0.88 for tabular extraction, surpassing or matching existing approaches. Application of the pipeline to over 10,000 articles yields the largest publicly available multicomponent alloy database and reveals compositional and processing-property trends. The database is further employed for sustainability-aware materials selection in three application domains, i.e., lightweighting, soft magnetic, and corrosion-resistant, identifying multicomponent alloy candidates with more sustainable production while maintaining or exceeding benchmark performance. The pipeline developed can be easily generalized to other class of materials, and assist in development of comprehensive, accurate and usable databases for sustainable materials design.

==> 0.abstract.tex <==
Machine learning (ML) methods have shown success in material design and optimization, but they rely on pre-existing, expensive, or manually curated datasets, limiting their potential for discovery. Natural language processing (NLP) methods, particularly large language models (LLMs), have been explored to extract materials data from literature corpus, but they often lack desired accuracy or are too narrow in their scope. In this work, we develop an LLM-based pipeline to accurately extract alloy-related information from both textual descriptions and tabular data in the literature. From textual sources, we extract various alloy details such as composition, processing conditions, characterization methods, and reported physical and mechanical properties. From tabular data, we extract alloy properties along with their corresponding units and values, supported by a comprehensive set of alloy properties commonly reported in high-entropy alloy (HEA) studies that we compiled. Our pipeline aims at increasing the sensitivity of LLMs to material domain knowledge which is vital to improve data extraction accuracy. We employ techniques such as prompt engineering (few-shot examples, context, roles, confirmations) and retrieval-augmented generation with various LLMs (GPT-4o, GPT-4omini, Llama-3, GPT-3.5 turbo) for this and achieved an F1-score of ~0.9 on textual data extraction and ~0.95 on tabular data extraction, significantly surpassing current models. We also developed evaluation methods to comprehensively assess the LLMs' performance, testing the pipeline against existing alloy datasets. The developed pipeline was applied to over 10,000 articles, producing the largest publicly available alloy dataset, and uncovering chemical trends such as correlations between alloy composition, mechanical properties, and processing conditions. The developed framework is quite versatile and can be used to develop LLMs for other material domains like polymers, metal-organic frameworks (MOFs), and ceramics. 

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
